Could you give me a hint? Generating inference graphs for defeasible reasoning

Defeasible reasoning is the mode of reasoning where conclusions can be overturned by taking into account new evidence. A commonly used method in cognitive science and logic literature is to handcraft argumentation supporting inference graphs. While humans find inference graphs very useful for reasoning, constructing them at scale is difficult. In this paper, we automatically generate such inference graphs through transfer learning from another NLP task that shares the kind of reasoning that inference graphs support. Through automated metrics and human evaluation, we find that our method generates meaningful graphs for the defeasible inference task. Human accuracy on this task improves by 20% by consulting the generated graphs. Our findings open up exciting new research avenues for cases where machine reasoning can help human reasoning. (A dataset of 230,000 influence graphs for each defeasible query is located at: https://tinyurl.com/defeasiblegraphs.)

==> sections/background.tex <==
\section{Background and tasks}
\begin{figure*}[!ht]
\centering
{\includegraphics[scale=0.5]{imgs/ig_comparison.pdf}}
\caption{\textbf{A} shows an Inference Graph adapted from \citep{Pollock2009ARS} (B) Influence Graph .}
\label{fig:igraph}
\end{figure*}

\subsection{Influence graphs}
\label{sec:igraphs}
Given a procedural text $T$, an influence graph~\citet{tandon2019wiqa} is an unweighted directed graph $G(V, E)$. 
A node $v \in V$ depicts an event (labeled with a short sentence or phrase) relevant to $T$.
The nodes in a graph belong to one of the following three categories:
a) nodes $\{\V{X}, \V{Y}, \V{W}\}$ depict changes to the events mentioned in the accompanying passage $T$.
b) nodes $\{\V{L}, \V{M}\}$ convey the accelerated or decelerated outcome caused of the events upstream in the graph,
and  finally, c) $\{\V{V}, \V{Z}, \V{U}\}$ are external events not mentioned in the passage $T$.

The edges between the nodes $v_i$ and $v_j$ captures the \textit{polarity} of the relation between them i.e. whether $v_i$ helps or hurts $v_j$.
Note that the polarity is transitively defined, and can be determined by traversing the graph between the events (e.g., \textit{virus becomes less contagious } \grn{helps} \textit{less virus enters the body}, \textit{virus becomes less contagious } \grn{hurts} \textit{more severe symptoms}).

\citet{tandon2019wiqa} released WIQA, a dataset of 2107 such influence graphs and the accompanying passages from a wide variety of domains including natural processes, physiology and working of everyday objects.
The edge structure in each graph takes one of two forms: $\V{X}\text{ helps }\V{M}$, where the path from node $\V{X}$ to node $\V{M}$ has a positive polarity, and $\V{X}\text{ hurts }\V{M}$, where the path has a negative polarity (as in Figure~\ref{fig:igraph}). 
The labels of the nodes $\{\V{Y}, \V{W}, \V{L}\}$ and the polarity of the associated edges also changes depending on whether the graphs is of type $\V{X}\text{ helps }\V{M}$ or $\V{X}\text{ hurts }\V{M}$.

\subsection{Defeasible Reasoning}

Defeasible reasoning is a type of commonsense reasoning that evaluates the likelihood of a hypothesis in the light of new evidence~\cite{rudinger-etal-2020-thinking}.
A defeasible reasoning query consists of three parts:
i) A premise \pre, that sets the context/background information (e.g., a contagious virus is spreading);
ii) A hypothesis \hypo, that posits a scenario relevant to the premise (e.g., person does not get sick); and
iii) An update \upd, which is an event that affects the hypothesis \hypo (e.g., wearing a mask).
The defeasible reasoning question is: \textit{Given a premise \pre, suppose an update event \upd happens. Does the update \upd \textbf{intensify} or \textbf{attenuate} the probability of a given hypothesis \hypo?}
For our example, given \pre, the event \upd \textbf{intensifies} the hypothesis \hypo.
In summary, each question comprises of a tuple \dques with a binary answer choice picked from \{\inten, \atten\}.

% For brevity, we refer to the labels intensifies and attenuates with +, - respectively and use the variable \utype to denote it.
% A complete defeasible reasoning query thus consists of \dquery.



==> sections/introduction-old.tex <==
\section{Introduction}
Humans often use background information to respond to a commonsense query.
Consider a question: \textit{Suppose a contagious respiratory virus is spreading. To avoid getting sick, should one wear a mask in public?} A typical response to this question would be a yes. 
On the surface, the impact of wearing a mask on avoiding sickness might be obvious.
However, to holistically reason about this scenario and explain this decision, it becomes important to think about events and facts that helped in reaching the conclusion: wearing a mask does not have a direct effect on the sickness, but it causes less virus to enter the body, thus reducing the chances of getting sick.
While such \textit{mediating} events are often used instinctively while dealing with commonsense situations, realizing them might help in contextualizing the decision.

Such mediating events play an especially important role in defeasible reasoning~\cite{rudinger-etal-2020-thinking}, a mode of reasoning that aims to judge the impact of an event~(e.g., wearing masks) on a hypothesis~(e.g., less sickness), in the context of a premise~(e.g., a contagious respiratory virus is spreading).
\citet{rudinger-etal-2020-thinking} derive a defeasible reasoning dataset~(\defeasible) from three varied phenomenon: commonsense reasoning~\cite{sap2019atomic}, social norms~\cite{forbes2020social}, and natural language inference~\cite{bowman2015large}.
Each sample in \defeasible consists of an update event \upd, a premise \pre, and a hypothesis \hypo.
The update \upd either intensifies or attenuates the the hypothesis \hypo.
The dataset only specifies the type of the type of the update; the reason for the relationship between the update \upd and the hypothesis \hypo is not specified.
% In other words, the query was tackled using (implicit) background knowledge (or commonsense). 
% In this scenario, this background knowledge was used in the form of a graph, where the nodes of the graph are the events of interest, and the edges indicate the nature of influence one event has on another (Figure 1).

% We posit that kind of background reasoning is not limited to the example that we have shown and is applicable to a wide range of everyday situations; while making decisions, we always think about the underlying and related events, and the way in which these events affect each other.
% As an oversimplification, one could imagine some sort of a graph that helps us in making these decisions. 
% Such a graph would involve one node for each potential event, and would capture the dependencies between these events in terms of cause, capturing how one event \textit{influences} another.
% This event influence graph, in conjunction with the passage, can help us in reasoning about the impact of one event on the other, and can further help us in evaluating the impact of a node on the other several reasoning hops away.
% Importantly, if we had access to such a graph, it would help us in capturing the dependencies between the events, and in potentially explaining the reason for the replies to any given commonsense query.

In this paper, we explore the possibility of generating background information that can rationalize and contextualize the response to a commonsense query.
Specifically, we seek to answer two research questions.
First, given a commonsense query, can we generate relevant background information that captures more context around the decision? For our example of wearing a mask to prevent sickness, this would involve generating a mediating event that mask prevents virus from entering the body, hence preventing sickness.
Second, is the rationale or context around a commonsense query helpful for humans? That is, does this machine generated context help humans in improving at their performance at the task?



We use large-scale pre-trained language models to generate background information for a given commonsense situation in the form of a graph. 
We use \wiqa~\cite{tandon2019wiqa} a dataset that provides event influence graphs grounded in a procedural passage.
We leverage methods in controllable text generation to encode the \wiqa corpus in a form that can be used to transfer the information to generate context for commonsense queries on other domains. 
We then generate such an influence graph for 230,000 defeasible reasoning queries~\cite{rudinger-etal-2020-thinking}, and conduct  human evaluation for the generated context graphs.
Our analysis shows that X\% of the explanations completely rationalize the commonsense query, and Y\% are highly-relevant.

% This brings us to the questions that we ask in this paper: i) Given a commonsense query, can the large pre-trained language models generate relevant background information used for answering commonsense queries, giving useful reasoning paths? and ii) Does such background information help the downstream performance of such QA models?
We take first steps towards answering these questions with the following contributions:
\begin{enumerate}
    \item We present a method to obtain additional information for each defeasible query in the form of an influence graph. We release a large dataset of 230,000 influence graphs accompanying each defeasible queries for further research.
    \item Our exhaustive human evaluation shows that humans perform better on defeasible inference (X\% by accuracy) when they are supplied with an influence graph with each defeasible query.
\end{enumerate}


==> sections/todo_notes.tex <==

\section{TODOs}



% \paragraph{Important questions to address:}
% \red{\begin{enumerate}
% \item Explanation vs. augmentation. We can these augmented knowledge, context, clarifications, but NOT explanation. We don't really know if Y explains Upd $\rightarrow$ H. \nk{Contextualize the input, and propose mediators to support reasoning}
% \item \sout{Why did you chose WIQA influence graphs and not some other way of obtaining these explanations?}
% \nk{Provides a structure that supports mediators and contextualization.  (mapping of update to X, hypo to L/M, premise to passage)}
% \item \sout{Methodology 
% Describe how you generate influence graphs for a defeasible query.}
% \item \sout{Clear explanation of the human eval, stress that we have the same evaluator pool.}
% \item \sout{What is the human baseline? Highlight that because of our special setup, we have a baseline (i.e., prior human eval).}
% \item \sout{Do these graphs also help the machines? Our focus in this paper is to find out if machine generated graphs help humans. This is future work.}
% \item \sout{Do some significance/hypo testing. (statistical significance -- what sample we chose).}
% \item \sout{Results (show few tables and show graphs)}
% \end{enumerate}}





\paragraph{questions to address:}

\red{\begin{enumerate}
\item \sout{I actually understood some of them after checking the appendix and WIQA paper Maybe providing more background on WIQA would help.}
\item  In Figure 1 , It is not clear why there is only C+ in the inference graph a, and both C+ and C- in graph (b). It is not clear why there should be two of them in this figure (You only focused on b for experiments, right?). Similarly, there is S+ and S- in graph a but  S and S- in graph b. (Solution: add figure 1b in middle for "adapted inference graph" and use it interchangeably in the paper)
\item  How is the positivity or negativity of contextualizer defined? Are they with respect to the hypothesis? For example in the output graph exemplified in appendix, why “less minerals in the soil” is C+? (Solution: it has a positive influence on the node it is connected with indicated by green, and C- would have a negative influence on the node indicated by red.)
\item  \sout{both contextualizers and mediators are generated during graph generation step. Also, the input only includes S, however the generated graph has both S, and S-? So how would it be different for defeasible task input where it has both S+ and S- ? aman: The input for defeasible will not have both}.
\item  \sout{I think it would be good if you could also include an input example to graph generator for defeasible inference (both strengthener and weakener) aman: added reference to the appendix .}
\item  Line 281: Why only keep strengthening contextualizer and mediators? Wouldn’t it hurt the prediction of weakener label in some ways? why not including both strengthener and weakener or randomly keep either + or -?
\item  Line 217: Just to follow the original notation, each DI inputs is (P, H, U)
\item \sout{Line 246: any citation for Struct-Match? how is Struct-MATCH calculated? A score of 97.63 means, it sounds like it’s almost perfect graph generation, yes?}
\item  Elaborate on the inference process, e.g. explaining a walk in the graph (in Figure 1(b) or Figure 2). 
\item  \sout{Shouldn’t the first line be   “Virus is more contagious” -> [more] -> “Wear a mask”?  Or am I misunderstanding C+ C-?}
\item  Cite Rationale Generation task on defeasible inference by Faeze Brahman. We addressed this rationale generation from a different angle.
\item The EMNLP paper’s IG terminology of contextualizers, situations, hypothesis, mediators isn’t from him, so the citation in Section 4 is a little bit misleading. Pollock is vague about the semantics of the graphs so doesn’t quite say what the leaf nodes mean. 
>> A2: We can be more explicit about these terminologies in Sec 4. 
\item it’s not really true to cite Pollock as a Cog Sci reference, he’s a formal logic person.  
\url{https://onlinelibrary.wiley.com/doi/abs/10.1207/s15516709cog1104_4} this is a cogsci journal so we can cite this instead. Though his paper is more logic and doesn’t mention cog-sci. >> A0: we can cite this cogsci journal paper
\item So if that’s true, then IGs don’t match Pollock’s scheme, although there’s other formalisms for argumentation that would easily match, e.g., with strengthener and weakener edges. e.g., from a quick Web search Pete found the formalism that might fit is Argument Map.
>> A4: Argument Map i.e. the diagram in Q6 will become incompatible with WIQA. We can add a line in related work that in order to adapt inference graphs and argument map like formalism to NLP, we make some relaxing assumptions so they map to existing NLP datasets.
\item \sout{The graphs from Could you Give Me A Hint? paper again seem mis-formed, e.g.,
what is the meaning of the link from  “S-: Robert doesn’t hallucinate”  to  “M-: “hallucinations are deceptive”? M- here is simply a fact, there’s no inferential or causal link from S- to M-.
Similarly from S+ to M+ : we want to show a conjunction: C+ \& M+ -> H rather than a chain.
C+ “people say truth generally [AND] Rob says elephant is pink” shouldn’t this be [AND] not [OR]
 A5: We will fix this example. (S+M+ point not clear) (M- can be hallucinations deceive people) (it should be [AND])
I think a reviewer in the rebuttal also pointed something in this example. The nodes can be like follows (bold shows changed nodes):
C+ : people say truth generally and Rob says elephant is pink
S+ elephant has mutated genes
S- Rob doesn’t hallucinate 
M+ : mutated genes change color
M- : hallucinations deceive Rob 
H: The elephant beside Rob is pink
Perhaps use diagram from Google doc on Peter's questions.}
\end{enumerate}}

%link: https://docs.google.com/document/d/1UAIMRtTXLBNLKXZG2uIV_Cy34uu2H-0ji3V-YEJw5GA/edit

% \todo{\paragraph{How can we be sure that the graphs were the main reason why annotators answered the queries better?}
% \begin{enumerate}
%     \item  First, in order to establish any gains over [2], we want to clarify that our setup is comparable to [2] because we sample an equal mix of questions from the test set of [2], where humans failed and where they succeeded (L269-280). We also ensure that the annotators are from precisely the same qualified pool as [2]. Further, the instruction set was imported as-is from [2], with the only additions being related to using the inference graph as additional information. We provide details of our experimental setup in the appendix (sample input-output Appendix A, Instructions to the annotators - Appendix C). This setup ensures that when we provide inference graphs to the annotators, any gains will be comparable to [2]. 
% \item Second, having established a comparable setup, we show significant gains in human performance due to adding inference graphs. We rely on a large number of questions and annotators to cancel out any noise introduced by effects caused due to shuffling or the annotator bias (500 questions, annotators sampled from a pool of 230 reviewers). We find that for over 22\% of the questions that were previously incorrectly answered were answered correctly using graphs (Figure 3). Crucially, for 40\% of these cases, the annotators marked that the graphs were helpful (compared to only 8\% graphs being helpful when their response was previously correct and now wrong) -- we will add these statistics in the next version. Finally, we find that the gains are statistically significant~(Table 4).
% Importantly, the annotators had a choice.
% \end{enumerate}}
